Higher Criticism to Compare Two Large Frequency Tables, with sensitivity to Possible Rare and Weak Differences

We adapt Higher Criticism (HC) to the comparison of two frequency tables which may -- or may not -- exhibit moderate differences between the tables in some unknown, relatively small subset out of a large number of categories. Our analysis of the power of the proposed HC test quantifies the rarity and size of assumed differences and applies moderate deviations-analysis to determine the asymptotic powerfulness/powerlessness of our proposed HC procedure. Our analysis considers the null hypothesis of no difference in underlying generative model against a rare/weak perturbation alternative, in which the frequencies of $N^{1-\beta}$ out of the $N$ categories are perturbed by $r(\log N)/2n$ in the Hellinger distance; here $n$ is the size of each sample. Our proposed Higher Criticism (HC) test for this setting uses P-values obtained from $N$ exact binomial tests. We characterize the asymptotic performance of the HC-based test in terms of the rarity parameter $\beta$ and the perturbation intensity parameter $r$. Specifically, we derive a region in the $(\beta,r)$-plane where the test asymptotically has maximal power, while having asymptotically no power outside this region. Our analysis distinguishes between cases in which the counts in both tables are low, versus cases in which counts are high, corresponding to the cases of sparse and dense frequency tables. The phase transition curve of HC in the high-counts regime matches formally the curve delivered by HC in a two-sample normal means model.

==> figure_tables.tex <==
\begin{figure}
    \centering
    % \begin{tikzpicture}
    % \node at (0,0) {
    % \includegraphics[scale=0.25]{Figs/pval_grid_exact_test.png}};
    % \end{tikzpicture}
    %
    \begin{tikzpicture}
    \node at (0,0) {\includegraphics[scale=0.6]{Figs/cont_table_col_dense.png}};
    \node at (6,0) 
    {\includegraphics[scale=0.6]{Figs/cont_table_hist_dense.png}};
    \end{tikzpicture}
    
    \begin{tikzpicture}
    \node at (0,0) {\includegraphics[scale=0.6]{Figs/cont_table_col_sparse.png}};
    \node at (6,0) 
    {\includegraphics[scale=0.6]{Figs/cont_table_hist_sparse.png}};
    \end{tikzpicture}
    
    \caption{
    Example of two-sample data under the null hypothesis in the $\dense$ and $\sparse$ cases. The number of occurrences of the $i$-th category is $\Pois(nP_i)$ in each sample.
    The baseline rates $(P_1,\ldots,P_N)$ are of Zipf-Mandelbrot with $\xi=0.4$ and $k=10$. The parameter $n$ is $8000$ in the top panels and $500$ in the bottom panels, corresponding to the cases $\dense$ and $\sparse$, respectively. 
    %
    Left panels: number of occurrences of each category in each coordinate and its expected value $nP_i$ (gray curve). Right panels: histogram of counts with category labeling removed. The color of the cell $(x,y) \in \mathbb N \times \mathbb N$ depicts the number of categories with counts $x_i=x$ and $y_i=y$.}
    \label{fig:tables}
\end{figure}

\iffalse
Figure~\ref{fig:pvals_exact} illustrates the function $\pi(x,y)$ in the range $x,y\in\{0,\ldots,25\}^2$. \par
\begin{figure}
    \centering
    \begin{tikzpicture}
    \node at (0,0) {\includegraphics[scale=0.5]{Figs/cont_table_hist_pvals_dense.png}};
    
    \node at (3.5,0) {\includegraphics[scale=0.5]{Figs/cont_table_hist_pvals_sparse.png}};
    
    \node at (8,0) {\includegraphics[scale=0.5]{Figs/pval_grid_exact_test.png}};
    \end{tikzpicture}
    \caption{Binomial P-values. The P-value associated with the coordinate 
    $(x,y)$ is the probability that the outcome of a binomial experiment with $n=x+y$ and $p=1/2$ is less probable than $x$. 
    %$\pi(x,y) = \Pr\left(|\Bin(x+y,1/2)-(x+y)/2)| \leq |x-y|/2\right)$: 
    }
    \label{fig:pvals_exact}
\end{figure}
\fi
